Scratch as Social Network: Topic Modeling and Sentiment Analysis in Scratch Projects

Societal matters like the Black Lives Matter (BLM) movement influence software engineering, as the recent debate on replacing certain discriminatory terms such as whitelist/blacklist has shown. Identifying relevant and trending societal matters is important, and often done using social network analysis for traditional social media channels such as twitter. In this paper we explore whether this type of analysis can also be used for introspection of the software world, by looking at the thriving scene of young Scratch programmers. The educational programming language Scratch is not only used for teaching programming concepts, but offers a platform for young programmers to express and share their creativity on any topics of relevance. By analyzing titles and project comments in a dataset of 106.032 Scratch projects, we explore which topics are common in the Scratch community, whether socially relevant events are reflected and how how the sentiment in the comments is. It turns out that the diversity of topics within the Scratch projects make the analysis process challenging. Our results nevertheless show that topics from pop and net culture in particular are present, and even recent societal events such as the Covid-19 pandemic or BLM are to some extent reflected in Scratch. The tone in the comments is mostly positive with catchy youth language. Hence, despite the challenges, Scratch projects can be studied in the same way as social networks, which opens up new possibilities to improve our understanding of the behavior and motivation of novice programmers.

==> content/relatedwork.tex <==
\section{Related Work}
\label{sec:rw}




==> content/resultsRQ1_Kopie.tex <==
\section{Results}
\subsection{RQ1: }
\label{sec:rq1}

\subsubsection{Analysis of Part of Speech}

%\begin{table}[tb]
%	\caption{Distribution of POS in code and project comments and meta-info (title, instructions, acknowledgements).}
%	\label{tab:pos}
%		\centering
%	   \begin{tabular}{l@{}rrrrrr}
%		\toprule
%		{} &
%		  \multicolumn{2}{c}{\textbf{Code comments}} &
%		  \multicolumn{2}{c}{\textbf{Meta-info}} &
%		  \multicolumn{2}{c}{\textbf{Project comments }} \\
%		  & {} & {\%} & {} & {\%} & {} & {\%} \\
%		  \midrule
%	   Noun  & 1.257.183 & 73.9  &    3.845.160 & 80.0  & 1.512.994  & 70.0  \\
%	   Verbs  & 213.251 & 12.5  &   419.641    & 8.6     & 262.504 & 12.2 \\
%	   Adjectives & 113.940 & 6.7  &  276.775 & 5.7    & 151.355 & 7.0   \\
%             Other & 115.480 & 6.9  & 294.937  & 5.7 & 213.026 & 10.8 \\
%             \midrule
%		Total  & 1.699.854 &  &  4.835.853 &  & 2.139.879 &   \\
%		\bottomrule
%	  \end{tabular}
%	\end{table}

As an initial step, we consider the distribution of POS in the code and project comments as well as meta-information including titles, instructions, and acknowledgements. 
Table~\ref{tab:pos} lists the most common grammatical paradigms in \Scratch projects. Three quarters of the code comments consist of nouns  74\%, while only 12.5\%are verbs and 6.7\% are adjectives. In the project comments, the situation is similar: They consist of about 70 \% nouns, 12.2 \% verbs and about 7\% adjectives. An intuitive expectation would have been that there are more adjectives in the project comments, similar to posts in social networks~\cite{guzmansentiment2014}, as adjectives in particular are representatives of emotions \cite{carterenglish2016} that appear essential in the reception of projects. 
In the meta-information almost 80 \% of all words are nouns. %(adjectives: \SI{5.7}{\%}, verbs: \SI{8.6}{\%}). 
This is due to the conception of a \textit{title}: Similar to media reports, concise nouns, nominalisation or ellipses in titles give a first impression of the content of a project. Articles and verbs are often left out \cite{carterenglish2016}. 
Since nouns represent content words, they are particularly suitable for topic analysis as they are adding contextual understanding. As project and code comments also contain many nouns, they have the potential to provide ample information for a thematic identification.

%Due to linguistic peculiarities of the dataset like acronyms or smileys, the specification may be distorted. Another special feature concerns the code comments: In these, many more numerals appear than in the other two categories.
%This can be explained by the fact that the code comments mostly contain instructions like \textit{waitfor5seconds}. Furthermore, numbers are part of the basic programming vocabulary and often used \textit{magic numbers} can be explained in the code comments. 

We also note differences in the overall word count per project. In projects where code comments are used, the total word count of code comments averages about 36 words. 
In contrast, the project comments of a project contain an average of about 19 words. This confirms the intuitive assumption that project comments contain shorter units, i.e., sentences. Project comments are unlikely to contain complex issues, but rather concise utterances \cite{thelwall2010sentiment}.

\summary{}{Predominantly nouns are used in all textual information of the projects, which potentially provide comprehensive semantic information.}

\subsubsection{Identification of semantic fields}\label{semanticfields}

%\begin{figure}[tb]
%	\centering
%	\includegraphics[width=\linewidth]{content/Pictures/codeAnalyse/topics/wordcloudTfidf23.pdf}
%	\caption{Weighted terms that appear in the meta-information of \Scratch projects. The term with the highest weight according to the tf-dif is displayed equivalently in the largest font size.}
%	\label{fig:tfidfwordcloud}
%\end{figure}

As a higher level of contextual understanding, the most frequent project terms are considered.
Fig. \ref{fig:tfidfwordcloud} shows the terms weighted by TF-IDF used in the meta-information (title, instructions and acknowledgements) of \Scratch projects. The highest weighting is achieved by the term \textit{spike ball}: A game of the genre \textit{Shoot 'em up}, where the avatar has to avoid mostly spiky or threatening objects (spike balls). %\footnote{While in reality spike ball is a combined sport of volleyball and 4square, spike ball in \Scratch refers to a classic \textit{Shoot 'em up}. This has been verified by a manual sighting.}
In general, some terms exist that refer to different common games: \textit{spin wheel}, \textit{dark soul}, \textit{space ball} or \textit{emoji maker}.

The term pairs \textit{space destroyer}, \textit{space invader}, \textit{star fighter}, \textit{star hunter} and \textit{space shoot} all refer to the subject \textit{space}.
Although the terms after \textit{space} differ in their word family, they belong together thematically and form the subject \textit{fight}.
The terms \textit{fight[er]}, \textit{shoot} and \textit{hunt[er]}---as representative of the characteristic of an active, violent act by at least two rival parties---can refer to the project type game. 
In addition, the reference \textit{space invader} is an indicator for this assumption---it represents one of the first video games that had a lasting influence on the gaming world.
Thus, the topic \textit{space invader} could be established already on the basis of the weighted terms.

However, some of the extracted terms are counterintuitively highly weighted: \textit{green flag}, \textit{arrow key}, or \textit{custom block} are almost obligatory instructions that can be found in many projects. This could be related to the fact that in some projects only one set of statements occurs and is therefore considered \textit{relevant} from an algorithmic perspective. 

%\begin{figure}[tb]
%	\centering
%	 \includegraphics[width=\linewidth]{content/Pictures/codeAnalyse/topics/wordcloudAllMetainfoText.pdf}
%	\caption{The most common terms \textbf{without} weighting in the meta-information: The influence of the absolute frequency is apparent as the majority of terms are of descriptive or instructive nature.}
%	\label{fig:tfidfwordcloudOHNE}
%\end{figure}

The counterpart to the illustration just shown is Fig.~\ref{fig:tfidfwordcloudOHNE}, which shows the most common terms of the meta-information \textbf{without} weighting. The discrepancy between absolute and weighted frequency becomes clear: Terms that define instructions such as \textit{click}, \textit{use}, \textit{press} or descriptions such as \textit{project} or \textit{remix} dominate the word cloud.
These expressions form the subject area of the instructions, which result from typical instructional texts such as \textit{press the green flag to play} or \textit{use the left and right arrows to move}. Although this terminology is interesting, it is irrelevant for the determination of concrete semantic fields.
%In addition to this distribution, the words that can provide information about certain concepts are also relevant: for example, the word \textit{player} is followed by the concept of a game, since this requires at least one player. 

%\begin{figure}[tb]
%	\centering
%	\includegraphics[width=\linewidth]{content/Pictures/codeAnalyse/topics/wordcloudCodeComments.pdf}
%	\caption{The most common terms in code comments without weighting: Besides statements like \textit{make} or \textit{change}, especially notations of the blocks like \textit{number} or \textit{block} itself are visible.}
%	\label{fig:codecommentswordcloud}
%\end{figure}

Fig. \ref{fig:codecommentswordcloud} shows how the frequency distribution behaves exclusively in the context of code comments. The majority of the terms represent mandatory statement notations like \textit{block}, \textit{make} or horizontal attributions like \textit{left} and \textit{right}.
The terms \textit{costume} and \textit{color}, which refer to an aesthetic component of the projects, are striking. The term \textit{clone} may refer to the programming concept or a cloned sprite.
In addition, it can be seen once again that with \textit{game}, \textit{level} and \textit{player} game-specific terminology is used.
Due to the frequency of statement notation, it seems that mainly descriptive statements are used in the code comments, which could also be derived from the semantics of the blocks without commenting.
This does not apply to the established correct use of code commenting, where especially the reason or particularities of code fragments should be given---not \textit{what} the code does, but \textit{why} \cite{martin2009clean}. This descriptive code comment is not just a problem for beginners: The concept is always the subject of controversial debates. 
The terminology of code comments considered here can provide information about the commenting behaviour of users and should be further researched, but they do not provide any added value for a semantic analysis.

%\begin{figure}[tb]
%	\centering
%	 \includegraphics[width=\linewidth]{content/Pictures/codeAnalyse/topics/wordcloudProjectComments.pdf}
%	\caption{The most frequent terms in project comments without weighting: Acronyms such as \textit{lol} or \textit{xd} and appreciative terms such as \textit{love} and \textit{thank [s/you]} are frequently used.}
%	\label{fig:projectcommentswordcloud}
%\end{figure}

Fig.~\ref{fig:projectcommentswordcloud} outlines the most common terms in project comments, and the context in which the terms are embedded is identifiable: 
Particular reference is made to emotionally connoted terms as well as acronyms that are offered in a social network~\cite{thelwall2010sentiment, rosenbaumoliverchatslang2001}. 
This manifests itself in expressions with an affective function such as \textit{love}, \textit{wow} or \textit{nice}. In addition, there seems to be an appreciative and honoring attitude (\textit{thank [s/you]}). 
Similar to code comments, the term \textit{game} stands out for its game-specific terminology. This could suggest the combination \textit{good game}. 
Other positively connoted terms like \textit{yeah}, \textit{cool} or \textit{well} can also be found. 
These affective terms are well suited for a sentiment analysis \cite{linSentiment2018}, but less for a topic determination and are therefore not considered for further analysis.

In particular, the acronyms \textit{lol} [laughing out loud] and \textit{xd} [xD, laughing face rotated by 90$^\circ$ degrees] refer to the user group as terms of net and youth jargon \cite{rosenbaumoliverchatslang2001}. 
These terms have established themselves in written communication as chat acronyms and serve as linguistic and cultural codes. These are also transferred to the non-virtual space \cite{noauthorlangenscheidt2011}, in which groups socialize. 
The terms belong to an age-related sociolect---through the use of a language system, assignment to a group is possible that is withheld from other persons (for example, \textit{older} persons). 
The language consists of certain signs and grammatical rules which are adhered to within the language groups. A deviation from these rules can not only be colloquial language or dialect, but also a (chat) acronym~\cite{desaussure1972}. 
These variants of the language are only comprehensible to those who know their codes and are themselves part of the same langue~\cite{desaussure1972}. This specific linguistic usage provides deeper understanding of the community of \Scratch, which should be deepened in further studies.

\summary{}{The most popular terms are domain-specific for each textual source: meta-information contains various topics, code comments consist mainy of instructions, and in project comments emotions and youth slang predominate. Therefore, meta-information is most promising for topic analysis. }


\subsubsection{Topic modeling}\label{topicmodeling}

\begin{table*}[tb!]
	\caption{Here the five most popular topics according to the LSA model are shown. As input all meta-information of the projects was evaluated with the parameters tf-idf k=(1,3) and LSA k=100. Besides the absolute number of projects belonging to a topic, five generated keywords with their weighting are shown.}
	\label{tab:topics}
	\begin{tabular}{@{}llllll@{}}
	\toprule
	\textbf{rank} & \textbf{\# projects} & \textbf{label}  & \textbf{keywords (weight)}  & \textbf{example ID} \\ \midrule
	1  & 47.259    & arcade game     & game (0.59), remix (0.34), maze (0.30), pong (0.19), arrow (0.16)    &    368496721 %379661384
	 \\
	2             & 25.902                      & starter project                                                & project (0.25), student (0.20), starter project (0.18), lesson (0.18), teacher lesson plan (0.10) &    378880117 % 383591657      
	 \\
	3             & 15.367                      & animation                                                      & make (0.31), fly (0.25), animation (0.22), click (0.18), space (0.18) &     357019003 %387290785      
	 \\
	4             & 7.786                       & ping pong                                                      & pong (0.55), remix (0.38), pong game (0.16), maze (0.10), ping pong (0.10)      &       357459447         \\
	5             & 6.821                       & adventure                                                      & task (0.41), adventure (0.28), button (0.20), summer (0.15), draw (0.09)&          385466467  %363773887, 377882545 
		\\
	%6             & 6.395                       & cat-mouse game     & cat (0.50), scratch (0.40), project (0.26), scratch project (0.13), mouse (0.12)      &   374472429  \\
	%7             & 6.211                       & instructions                                                   & flag (0.23), green flag (0.22), green (0.21), click (0.14), press green flag (0.14) &              358326480      \\
	%8             & 6.104                       & adventure & thing (0.22), character (0.22), adventure (0.21), war (0.16), downhill ski (0.13)      & 385758935 %fire and water reference 
	\\
	%9             & 5.878                       & instructions                                                   & flag (0.22), game (0.22), green flag (0.22), green (0.21), click (0.14)     &              356750670\\
	%10            & 5.767                       & jump 'n' run game                                                           & run (0.34), add (0.33), mario (0.19), jump (0.18), fly (0.17)      &   376584997  \\ 
	\bottomrule
	\end{tabular}
	\end{table*}

%	\begin{figure*}[tb]
%		\centering
%		\subfloat[\label{mario}\# 1: \textit{chomper remix v.2} \tiny(ID 368496721)]{\includegraphics[width=0.16\linewidth]{content/Pictures/manuelleAnalyse/chomper368496721.png}}\hfill
%		\subfloat[\label{watergirl}\# 1: \textit{Fireboy and Watergirl} \tiny(ID 379661384)]{\includegraphics[width=0.16\linewidth]{content/Pictures/manuelleAnalyse/watergirl379661384.png}}\hfill
%		\subfloat[\# 2: \textit{Interactive Art Starter Project - Dido Elizabeth Bell remix} \tiny(ID 378880117)]{\includegraphics[width=0.16\linewidth]{content/Pictures/manuelleAnalyse/starter378880117.png}}\hfill
%		\subfloat[\# 2: \textit{Dance Party Starter Project 1 remix} \tiny(ID 383591657)]{\includegraphics[width=0.16\linewidth]{content/Pictures/manuelleAnalyse/starter383591657.png}}\hfill
%		\subfloat[\label{bluestar}\# 3: \textit{Bluestar and Amberfur}\tiny(ID 357019003)]{\includegraphics[width=0.16\linewidth]{content/Pictures/manuelleAnalyse/animation357019003.png}}\hfill
%		\subfloat[\label{disney}\# 3: \textit{Disney Dress Up [updated] remix}\tiny(ID 387290785)]{\includegraphics[width=0.16\linewidth]{content/Pictures/manuelleAnalyse/disneyDressUp.png}}\hfill
%		\caption{The three most popular topics (Tab. \ref{tab:topics}) are shown, each with two randomly selected example projects.}
%		\label{fig:sampleTopics}
%	\end{figure*}

Only meta-information (title, instructions and acknowledgement) is included in the topic modeling as we determined that code and project comments distort the result of the occurrences of the context-specific terminology (\ref{semanticfields}). 

In Table \ref{tab:topics} the five most popular topics with their generated keywords from the LSA model and manually chosen labels are presented.
In this ranking, projects are assigned to the topic that is closest to the one in the matrix of the SVD~(\ref{svd}) and therefore, the topics and their distribution are only indicators~\cite{maleticusing2000}. Fig. \ref{fig:sampleTopics} gives an impression of example projects for the three most popular topics.

In these topics limitations of the model become apparent, as it mainly extracts keywords that can be assigned to categories or instructions and less \textit{real} semantic topics:
%
According to the result of the LSA model, the most popular topic in \Scratch projects is the project type arcade game. According to the \Scratch website, the type \textit{game} and its subcategories like \textit{maze} or \textit{pong} are the most popular project category in \Scratch.\footnote{https://en.scratch-wiki.info/wiki/Game\_Projects} This can be verified as most of the topics in the top-10 contain game-specific terminology like \textit{game}, \textit{run}, \textit{jump}.
The second most popular topic is filled with the keywords from the semantic field \textit{starter project}. This is due to the fact that \Scratch offers different pre-fabricated projects which help programming beginners to start programming projects.\footnote{https://scratch.mit.edu/starter-projects} As it is on the second place, the concept seems to be well received from the community.
In third place is again a topic related to project types: animation. Besides games, animations are another popular category in the \Scratch world.\footnote{https://en.scratch-wiki.info/wiki/Animation\_Projects}


\begin{table}[tb]
	\caption{Topics generated by the LSA model whose five keywords with the highest weight do not contain any terminology regarding the project category or instructions. Any duplication of terms (e.g. \textit{star, hunter, star hunter}) is due to the n-grams=(1,3). Topics related to the COVID-19 pandemic are highlighted.}
	\label{tab:topics25}
	\begin{tabular}{@{}ll@{}}
	\toprule
	\textbf{\# projects} & \textbf{keywords}                                                \\ \midrule
	6104        & thing, character,  adventure, war, downhill ski         \\
	5354        & shoot, button,  mario, world, zombie                    \\
	5354        & letter, task, love, end, sonic                          \\
	3958        & letter, day, food, change, sound                        \\
	3198        & dance, party, dance party, chase, music                 \\
	3036        & star, war, hunter, star hunter, star war                \\
	2719        & music, catch, music video, miner cat                    \\
	2624        & test, character, art, school, dance                     \\
	\rowcolor{lightgray}
	2461        & star, virus, simulator, mouse, star hunter              \\
	2448        & fish, little fish, mouse, little, eat                   \\ 
	2045        & birthday, summer, cake, birthday cake, binary birthday  \\
	1965        & flappy, bird, flappy bird, art, music                   \\
	1482        & paper, rock, rock paper, scissors, paper scissors       \\
	1249        & candy, paper, rock paper, scissors, paper scissors      \\
	1181        & fish, candy, earth day, little fish, clicker            \\
	1153        & hide seek, seek, hide, flashlight, flashlight hide seek \\
	971         & knight, choppy knight, choppy, summer, character        \\
	942         & alien explorer, alien, explorer, space, fly             \\
	\rowcolor{lightgray}
	873         & test, virus, sprite, simulator, final                   \\
	626         & ball, fly, space, miner cat, flappy                     \\
	585         & talent, musical talent, musical, race, villain          \\
	555         & dj, mixer, dj mixer, final, fish                        \\
	506         & quiz, dance, jump, mario, run, dinosaur                 \\
	469         & parcel, parcel express, express, rock, box          \\ \bottomrule
	\end{tabular}
	\end{table}

However, the LSA model also generated topics that add more
contextual understanding, which become more apparent when excluding
terminology regarding project categories or instructions. In addition to
the terms \textit{game},\textit{remix}, \textit{starter},
\textit{animation}, these include implicit terms such as \textit{make}
or \textit{click}. Table \ref{tab:topics25} lists the 24 topics whose five keywords
with the highest weight do not contain any of these terms.

%The opposition pair \textit{cat} versus \textit{mouse} appears as a game type in place 6. They belong to the collective noun \textit{animals}, which could also represent a thematic area. Such rudimentary cat-and-mouse games would be a good project for beginners as it is a common game type in \Scratch\footnote{https://en.scratch-wiki.info/wiki/Cat\_and\_Mouse}.
%One of the most common terms in the paradigm \textit{instructions} is \textit{green flag} and \textit{game} (rank 7 and 9), which indicates that these topics represents the instructions of games and interactive projects.

We note that intermedial and intertextual references to existing media products of pop culture such as \textit{pong} (rank 1 and 4, \ref{tab:topics}) as well as \textit{flappy bird} and \textit{mario} (\ref{tab:topics25}) exist, which indicates a reflection of well-known cultural games. Some example projects to emphasize this impression are \textit{Super Mario Bros.} (\ref{mario}), the Browser-game \textit{Fireboy and Watergirl in the Forest Temple}~(\ref{watergirl}), Erin Hunter's \textit{Warriors} (\ref{bluestar}) and Disney Princesses (\ref{disney}).
%An important observation regarding the keywords in each topic is that some words, such as \textit{game}, occur in several topics. This is an advantage of topic modeling in contrast to \textit{hard} cluster analyses: Topics used in natural language may overlap in terms of the words used. Likewise, terms like \textit{click} are context-independent.
%
Furthermore, two topics in Tab. \ref{tab:topics25} even contain terminology that can be attributed to the COVID-19 pandemic, indicated by the term \textit{virus}. Thus the topics also address social events, which will be discussed in more detail in RQ2.

\summary{}{The LSA model is dominated by references to \Scratch project categories, such as game and animation. %Pre-fabricated starter projects seem to be readily accepted from the community.
  However, reflections of pop culture and societal events exist, suggesting application of advanced semantic analyses.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

\summary{RQ1}{}

==> content/resultsRQ2.tex <==
\subsection{RQ2: Representation of Topics}
\label{sec:rq2}


The COVID-19 pandemic lends itself as an extra-discursive event: The term \textit{Corona} has been known mainly since the outbreak of the virus.\footnote{Before the pandemic, the term \textit{Corona} was associated mainly with the Mexican beer brand \textit{Corona Extra}.}
Analogous to social media analyses~\cite{abd2020top,wangpublic2020}, this section describes a trend analysis to determine how long and how many projects have been dealing with the keyword \textit{Corona}. 

\subsubsection{COVID-19 Trend Analysis}\label{trendanalyse}

%\begin{figure}[tb]
%  \centering
%  \subfloat[\label{fig:Corona} Distribution of \Scratch projects with the keyword \textit{Corona} by their release date. This is a clear reaction to the  events of the COVID-19 pandemic. The fall of the curve in April is due to the mining process, the fall in early May is related to the end of the mining period.]{
%    \includegraphics[width=\linewidth]{content/Pictures/codeAnalyse/topics/distributionCovid1000}
%    }\\
%  \subfloat[\label{fig:googleCorona} Distribution of the worldwide Google search query with the keyword \textit{Corona} according to their query date. Similar to \Scratch projects, a significant increase in the middle of March is observed.]{
%    \includegraphics[width=\linewidth]{content/figures/projects/googleCorona.png}
%  }
%    \caption{Trends related to the keyword \textit{Corona}.}
%\end{figure}

%In addition to the topics generated in \ref{topicmodeling}, some of the topics contain terminology around COVID-19. % but are not among the Top-10 topics. 
%The most popular of these (2,461 projects) contains the following terms in ascending order of weight: \textit{star, virus, simulator, mouse, star hunter, press, coronavirus}. Similarly, a topic (873 projects) is described by the keywords \textit{text, virus, sprite, simulator, final, mario, cat, coronavirus}. Another theme (414) is associated with the terms \textit{sprite, star, assignment, arrow, fish, race, attac, space, virus}. Similar to the findings from \ref{sectionRQ1}, it is noticeable that there are also irrelevant words like \textit{sprite} in addition to meaningful terms such as \textit{coronavirus} or \textit{star hunter}.

Fig.~\ref{fig:Corona} clearly shows a trend: A total of 1,800 projects of the entire data set contain the keyword \textit{Corona} by searching title, instructions and acknowledgements.
In direct comparison with the result of search query in Google Trends\footnote{https://trends.google.de/trends/explore?q=Corona}  in Fig.~\ref{fig:googleCorona}, the similarities in the trends are clearly visible.
Both Google query and \Scratch projects show a huge increase from early to mid March as this  was the period when the virus spread from Asia to Europe and America. On 11 March 2020, the World Health Organisation declared it as a pandemic, thereby shifting the public perception~\cite{cucinotta2020declares}. This was accompanied by an increase in media coverage, which in turn must be taken into account as an influencing factor.


\vspace{2mm}Given the clearly noticeable trend visible in the data, we turn to a manual investigation of \textit{how} \Scratch projects deal with the COVID-19 pandemic. 
Since the extraction of the semantic information in \ref{topicmodeling} showed that mainly project categories were identified, the manual analysis examines projects from the two apparently most popular categories, animations and games, for their reflection of the COVID-19 pandemic.

\subsubsection{COVID-19 as Animation}
\begin{figure*}[tb]
	\centering
	\subfloat[\label{fig:mask1}There is besides the graphic a textual description. One can interact by clicking the arrows forward or backward (ID 389852531).]{\includegraphics[width=0.30\linewidth]{content/figures/projects/mask.png}}
	\hfill
	\subfloat[\label{fig:mask2}A rather abstract instructions with rudimentary iconicity to a mask is shown. This is a pure animation without interaction (ID 397136809).]{\includegraphics[width=0.30\linewidth]{content/figures/projects/mask2.png}}
	\hfill
	\subfloat[\label{fig:mask3}In this project, a very authentic mask \textit{sewed}. To sew it, one has to click on the respective hole (ID 387096633).]{\includegraphics[width=0.30\linewidth]{content/figures/projects/mask3.png}}
	\caption{Analogue to other networks like YouTube,  Instagram or Twitter \cite{dumais1988using}, sewing instructions for masks are also passed on in \Scratch projects. These instructions vary not only in their complexity and abstraction, but also in their degree of interaction.}
	\label{fig:mask}
\end{figure*}

Similar to posts in social networks, where instructions for DIY masks as a protective manner became popular~\cite{dumais1988using},
 \Scratch projects also deal with this topic (Fig.~\ref{fig:mask}). This is surprising, since sewing instructions for masks in a programming language initially seems counterintuitive.
In this context, not only the similarity to social networks is striking, but also the different forms of instructions. 
At first, most of the instructions considered and illustrated here follow a clear linear process. 
In the implementation the visual component is then abstracted---from rudimentary iconic masks to detailed and authentic representation with indexical form.

Power and hegemony around social positions is also presented, which is always provided with meaning~\cite{foucault1978dispositive}---if a sewing instruction is constructed, this also means that the project creator is a proponent of using masks and is aware of their protective mechanism. This is also one of the main topics which are observed in social media analysis~\cite{dumais1988using}.
The sewing of masks is legitimized (by authorities) and thus fits into a sociopolitical discourse. In this way, the person---depending on the feelings of the respective authorities---is integrated as a disruptive or civil society supporter. 
\Scratch projects thus find themselves in a collaborative role to the state and society.


\subsubsection{COVID-19 as Game}

\begin{figure*}[tb]
	\centering
	\subfloat[\label{fig:corona1}In the game, the shield appears as an icon to obtain a protective item.]{\includegraphics[width=0.30\linewidth]{content/figures/projects/corona.png}}
	\hfill
	\subfloat[\label{fig:corona2}This \textit{protective equipment} represents a face mask when the shield is collected twice.]{\includegraphics[width=0.30\linewidth]{content/figures/projects/corona2.png}}
	\hfill
	\subfloat[\label{fig:corona3}After the third pick up of the shield, an \textit{armour} and three lives more is acquired.]{\includegraphics[width=0.30\linewidth]{content/figures/projects/corona3.png}}
	\hfill
	\caption{The project \textit{Corona Virus Simulator} is about the fight against the virus, whereby the goal is to avoid the virus. Thereby, one can also acquire protective equipment such as face masks, similar to reality.}
	\label{fig:coronaGame}
\end{figure*}

One of the most popular projects on the platform with almost 190,000 views (as of October 2020) that approaches the topic in a very \textit{interactive} mode is the project \textit{Corona Virus Simulator} (ID: 375802116). The project contains not only a reference to the concept of \textit{spike ball} in \ref{semanticfields}, but matches also keywords from the topic modeling in Tab. \ref{tab:topics25}. It is a classic representative of the \textit{Bullet Hell} genre, a subgenre of the \textit{Shoot 'em up} genre. The avatar has to avoid the oncoming viruses. 
This representation of a virus is an icon: The subjects in the game share the characteristics of a virus in reality. These include the capsid form and the negative connotation of virus as \textit{evil} or \textit{bad}, which is illustrated by the \textit{evil}-looking face. Likewise, the Avatar's power of action is limited---they cannot actively defend themselves with weapons, for example.

Similar to classic \textit{Bullet Hell} games, the Avatar's vulnerability manifests itself in a loss of \textit{life} (game attempts). 
Thereby, the Avatar's chances of survival (more lives) can be increased by several protective equipment items. Picking up an iconic shield increases the number of lives. 
Significant is the representation of the protective equipment as eye and mouth protection. In this context, an equation is established: Similar to reality in which wearing of face mask has a protective effect, the wearing of just this iconic protective equipment means higher chances of survival in the depicted world. 
%It is interesting here that it is not explicitly mentioned that protective equipment exists and what function it has. 
%The game mechanism alone---when collecting a shield, face and eye mask are displayed---opens up this level of meaning. 
It is also interesting how the topic COVID-19 is dealt with here: (1) it is a classic hero/antagonist game; (2) it differs from reality in an improper, i.e., ironic way by saying in the manual that it is a \textit{super accurate Corona virus simulator}, where evasion as well as protective equipment are essential; and (3) it is interesting that the notes point out the seriousness of Covid as a disease (\textit{ATTENTION: Covid-19 is a very serious illness and should be taken seriously.}) and even provide a link to the prevention page with an overview of the symptoms.


\summary{RQ2}{Similar to Google Trends, \Scratch projects with the topic COVID-19 increased in March 2020. Similar to social networks, instructions for DIY masks were implemented in \Scratch animations. The fight against COVID-19 is staged in \Scratch games as a classic shooter.}


==> content/resultsRQ2_Kopie.tex <==
\subsection{RQ2: Representation of topics}
\label{sec:rq2}


The COVID-19 pandemic lends itself as an extra-discursive event: The term \textit{Corona} has been known mainly since the outbreak of the virus.\footnote{Before the pandemic, the term \textit{Corona} was associated mainly with the Mexican beer brand \textit{Corona Extra}.}
Analogous to social media analyses~\cite{abd2020top,wangpublic2020}, this section describes a trend analysis to determine how long and how many projects have been dealing with the keyword \textit{Corona}. 

\subsubsection{COVID-19 Trend Analysis}\label{trendanalyse}

%\begin{figure}[tb]
%  \centering
%  \subfloat[\label{fig:Corona} Distribution of \Scratch projects with the keyword \textit{Corona} by their release date. This is a clear reaction to the  events of the COVID-19 pandemic. The fall of the curve in April is due to the mining process, the fall in early May is related to the end of the mining period.]{
%    \includegraphics[width=\linewidth]{content/Pictures/codeAnalyse/topics/distributionCovid1000}
%    }\\
%  \subfloat[\label{fig:googleCorona} Distribution of the worldwide Google search query with the keyword \textit{Corona} according to their query date. Similar to \Scratch projects, a significant increase in the middle of March is observed.]{
%    \includegraphics[width=\linewidth]{content/figures/projects/googleCorona.png}
%  }
%    \caption{Trends related to the keyword \textit{Corona}.}
%\end{figure}

%In addition to the topics generated in \ref{topicmodeling}, some of the topics contain terminology around COVID-19. % but are not among the Top-10 topics. 
%The most popular of these (2,461 projects) contains the following terms in ascending order of weight: \textit{star, virus, simulator, mouse, star hunter, press, coronavirus}. Similarly, a topic (873 projects) is described by the keywords \textit{text, virus, sprite, simulator, final, mario, cat, coronavirus}. Another theme (414) is associated with the terms \textit{sprite, star, assignment, arrow, fish, race, attac, space, virus}. Similar to the findings from \ref{sectionRQ1}, it is noticeable that there are also irrelevant words like \textit{sprite} in addition to meaningful terms such as \textit{coronavirus} or \textit{star hunter}.

Fig.~\ref{fig:Corona} clearly shows a trend: A total of 1,800 projects of the entire data set contain the keyword \textit{Corona} by searching title, instructions and acknowledgements.
In direct comparison with the result of search query in Google Trends\footnote{https://trends.google.de/trends/explore?q=Corona}  in Fig.~\ref{fig:googleCorona}, the similarities in the trends are clearly visible.
Both Google query and \Scratch projects show a huge increase from early to mid March as this  was the period when the virus spread from Asia to Europe and America. On 11 March 2020, the World Health Organisation declared it as a pandemic, thereby shifting the public perception~\cite{cucinotta2020declares}. This was accompanied by an increase in media coverage, which in turn must be taken into account as an influencing factor.


\summary{}{Similar to Google Trends, \Scratch projects with the topic COVID-19 increased in March 2020. }


\vspace{2mm}Given the clearly noticeable trend visible in the data, we turn to a manual investigation of \textit{how} \Scratch projects deal with the COVID-19 pandemic. 
Since the extraction of the semantic information in \ref{topicmodeling} showed that mainly project categories were identified, the manual analysis examines projects from the two apparently most popular categories, animations and games, for their reflection of the COVID-19 pandemic.

\subsubsection{COVID-19 as Animation}
\begin{figure*}[tb]
	\centering
	\subfloat[\label{fig:mask1}There is besides the graphic a textual description. One can interact by clicking the arrows forward or backward (ID 389852531).]{\includegraphics[width=0.30\linewidth]{content/figures/projects/mask.png}}\hfill
	\subfloat[\label{fig:mask2}A rather abstract instructions with rudimentary iconicity to a mask is shown. This is a pure animation without interaction (ID 397136809).]{\includegraphics[width=0.30\linewidth]{content/figures/projects/mask2.png}}\hfill
	\subfloat[\label{fig:mask3}In this project, a very authentic mask \textit{sewed}. To sew it, one has to click on the respective hole (ID 387096633).]{\includegraphics[width=0.30\linewidth]{content/figures/projects/mask3.png}}
	\caption{Analogue to other networks like YouTube,  Instagram or Twitter \cite{dumais1988using}, sewing instructions for masks are also passed on in \Scratch projects. These instructions vary not only in their complexity and abstraction, but also in their degree of interaction.}
	\label{fig:mask}
\end{figure*}

Similar to posts in social networks, where instructions for DIY masks as a protective manner became popular~\cite{dumais1988using},
 \Scratch projects also deal with this topic (Fig.~\ref{fig:mask}). This is surprising, since sewing instructions for masks in a programming language initially seems counterintuitive.
In this context, not only the similarity to social networks is striking, but also the different forms of instructions. 
At first, most of the instructions considered and illustrated here follow a clear linear process. 
In the implementation the visual component is then abstracted---from rudimentary iconic masks to detailed and authentic representation with indexical form.

Power and hegemony around social positions is also presented, which is always provided with meaning~\cite{foucault1978dispositive}---if a sewing instruction is constructed, this also means that the project creator is a proponent of using masks and is aware of their protective mechanism. This is also one of the main topics which are observed in social media analysis~\cite{dumais1988using}.
The sewing of masks is legitimized (by authorities) and thus fits into a sociopolitical discourse. In this way, the person---depending on the feelings of the respective authorities---is integrated as a disruptive or civil society supporter. 
\Scratch projects thus find themselves in a collaborative role to the state and society.

\summary{}{Similar to social networks, instructions for DIY masks were implemented in \Scratch animations.}

\subsubsection{COVID-19 as Game}

\begin{figure*}[tb]
	\centering
	\subfloat[\label{fig:corona1}In the game, the shield appears as an icon to obtain a protective item.]{\includegraphics[width=0.30\linewidth]{content/figures/projects/corona.png}}\hfill
	\subfloat[\label{fig:corona2}This \textit{protective equipment} represents a face mask when the shield is collected twice.]{\includegraphics[width=0.30\linewidth]{content/figures/projects/corona2.png}}\hfill
	\subfloat[\label{fig:corona3}After the third pick up of the shield, an \textit{armour} and three lives more is acquired.]{\includegraphics[width=0.30\linewidth]{content/figures/projects/corona3.png}}\hfill
	\caption{The project \textit{Corona Virus Simulator} is about the fight against the virus, whereby the goal is to avoid the virus. Thereby, one can also acquire protective equipment such as face masks, similar to reality.}
	\label{fig:coronaGame}
\end{figure*}

One of the most popular projects on the platform with almost 190,000 views (as of October 2020) that approaches the topic in a very \textit{interactive} mode is the project \textit{Corona Virus Simulator} (ID: 375802116). The project contains not only a reference to the concept of \textit{spike ball} in \ref{semanticfields}, but matches also keywords from the topic modeling in Tab. \ref{tab:topics25}. It is a classic representative of the \textit{Bullet Hell} genre, a subgenre of the \textit{Shoot 'em up} genre. The avatar has to avoid the oncoming viruses. 
This representation of a virus is an icon: The subjects in the game share the characteristics of a virus in reality. These include the capsid form and the negative connotation of virus as \textit{evil} or \textit{bad}, which is illustrated by the \textit{evil}-looking face. Likewise, the Avatar's power of action is limited---they cannot actively defend themselves with weapons, for example.

Similar to classic \textit{Bullet Hell} games, the Avatar's vulnerability manifests itself in a loss of \textit{life} (game attempts). 
Thereby, the Avatar's chances of survival (more lives) can be increased by several protective equipment items. Picking up an iconic shield increases the number of lives. 
Significant is the representation of the protective equipment as eye and mouth protection. In this context, an equation is established: Similar to reality in which wearing of face mask has a protective effect, the wearing of just this iconic protective equipment means higher chances of survival in the depicted world. 
%It is interesting here that it is not explicitly mentioned that protective equipment exists and what function it has. 
%The game mechanism alone---when collecting a shield, face and eye mask are displayed---opens up this level of meaning. 
It is also interesting how the topic COVID-19 is dealt with here: (1) it is a classic hero/antagonist game; (2) it differs from reality in an improper, i.e., ironic way by saying in the manual that it is a \textit{super accurate Corona virus simulator}, where evasion as well as protective equipment are essential; and (3) it is interesting that the notes point out the seriousness of Covid as a disease (\textit{ATTENTION: Covid-19 is a very serious illness and should be taken seriously.}) and even provide a link to the prevention page with an overview of the symptoms.

\summary{}{The fight against COVID-19 is staged in \Scratch games as a classic shooter.}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


\summary{RQ2}{}


==> content/tables/topictable_Kopie.tex <==
\begin{table*}[tb]
\centering
\footnotesize
\label{tab:topics}
\caption{Automatically generated topics from the Top2Vec model with their keywords and project statistics.}
\begin{tabular}{lp{13cm}rrrr}
\toprule
{ID} &             keywords (score) & \# views & \# loves & \# fav. &  \# pro. \\
\midrule
0     &                                         un (0.57) idk (0.56) way (0.54) ya (0.53) le (0.52) one (0.52) dude (0.51) au (0.5) dont (0.5) en (0.5) &      2859993 &       184844 &           146127 &       29552 \\
1     &  covid (0.52) sharkyshar (0.51) pfp (0.51) stickmin (0.5) tvokids (0.5) funkin (0.44) oyunu (0.42) numberblock (0.41) gacha (0.39)  &        49850 &         4454 &             3510 &        1062 \\
5     &                  cat (0.81) kitty (0.74) chat (0.63) pet (0.44) animal (0.41) mouse (0.4) bunny (0.39) dog (0.38) hedgehog (0.38) monkey (0.38) &        39033 &         3269 &             2507 &         632 \\
%7     &               mario (0.42) drew (0.42) henry (0.39) taco (0.36) angel (0.35) pico (0.35) corona (0.33) spongebob (0.33) pac (0.32) rylee (0.32) &        20830 &         1907 &             1393 &         521 \\
%14    &        song (0.78) music (0.51) sings (0.48) lyric (0.47) sing (0.46) playlist (0.45) nutshell (0.45) musical (0.43) rp (0.42) nightcore (0.41) &        32967 &         2187 &             1751 &         390 \\
22    &      mario (0.87) pokemon (0.45) kirby (0.43) minecraft (0.41) pong (0.39) sonic (0.38) spongebob (0.38) lego (0.37) tycoon (0.37)  &       122897 &         3020 &             2564 &         346 \\
27    &                                    lol (0.89) omg (0.83) xd (0.8) wow (0.76) oh (0.72) ay (0.71) funny (0.69) ya (0.69) dude (0.68) cool (0.67) &        12273 &         1140 &              771 &         315 \\
28    &               music (0.85) musical (0.62) song (0.59) rap (0.52) playlist (0.49) band (0.49) sings (0.47) rock (0.46) piano (0.44) dance (0.44) &        14624 &          993 &              846 &         262 \\
37    &             pong (0.71) ping (0.56) ball (0.38) duck (0.36) balloon (0.35) basketball (0.35) tv (0.33) soccer (0.32) piggy (0.32) orange (0.32) &         6625 &          507 &              410 &         230 \\
43    &           potter (0.78) harry (0.64) pokemon (0.41) disney (0.37) avatar (0.34) magic (0.34) maze (0.33) cake (0.31) book (0.3) minecraft (0.3) &         8408 &         1067 &              816 &         212 \\
45    &          adventure (0.87) journey (0.5) mystery (0.44) fun (0.44) maze (0.43) life (0.42) quest (0.42) avatar (0.42) trail (0.42) escape (0.41) &        33738 &         1831 &             1477 &         209 \\
51    &             space (0.83) rocket (0.51) moon (0.48) alien (0.46) galaxy (0.46) planet (0.41) earth (0.4) fighter (0.39) fight (0.39) wing (0.39) &         9229 &          649 &              544 &         198 \\
61    &   quiz (0.82) test (0.44) answer (0.33) favorite (0.31) alphabet (0.31) qa (0.31) imposter (0.31) question (0.31) match (0.29) challenge (0.29) &         8609 &          709 &              532 &         179 \\
85    &            zombie (0.92) dead (0.44) halloween (0.44) coffin (0.42) alien (0.4) ghost (0.39) shooter (0.39) gun (0.37) crash (0.37) hunt (0.37) &         9519 &          531 &              448 &         150 \\
87    &  dragon (0.85) pokemon (0.45) godzilla (0.44) wing (0.43) dinosaur (0.42) dungeon (0.42) monkey (0.42) snake (0.41) rocket (0.41)  &         5539 &          528 &              401 &         147 \\
90    &    christmas (0.84) santa (0.57) merry (0.54) winter (0.48) halloween (0.46) birthday (0.42) gift (0.4) party (0.36) potter (0.35) candy (0.34) &         9537 &         1049 &              790 &         145 \\
99    &            rainbow (0.84) balloon (0.41) sky (0.4) unicorn (0.4) neon (0.4) purple (0.39) cloud (0.37) dragon (0.36) shark (0.35) pink (0.35) &         7803 &          697 &              543 &         136 \\
\bottomrule
\end{tabular}
\end{table*}
